Force-Ultrasound Fusion: Bringing Spine Robotic-US to the Next "Level"

Spine injections are commonly performed in several clinical procedures. The localization of the target vertebral level (i.e. the position of a vertebra in a spine) is typically done by back palpation or under X-ray guidance, yielding either higher chances of procedure failure or exposure to ionizing radiation. Preliminary studies have been conducted in the literature, suggesting that ultrasound imaging may be a precise and safe alternative to X-ray for spine level detection. However, ultrasound data are noisy and complicated to interpret. In this study, a robotic-ultrasound approach for automatic vertebral level detection is introduced. The method relies on the fusion of ultrasound and force data, thus providing both "tactile" and visual feedback during the procedure, which results in higher performances in presence of data corruption. A robotic arm automatically scans the volunteer's back along the spine by using force-ultrasound data to locate vertebral levels. The occurrences of vertebral levels are visible on the force trace as peaks, which are enhanced by properly controlling the force applied by the robot on the patient back. Ultrasound data are processed with a Deep Learning method to extract a 1D signal modelling the probabilities of having a vertebra at each location along the spine. Processed force and ultrasound data are fused using a 1D Convolutional Network to compute the location of the vertebral levels. The method is compared to pure image and pure force-based methods for vertebral level counting, showing improved performance. In particular, the fusion method is able to correctly classify 100% of the vertebral levels in the test set, while pure image and pure force-based method could only classify 80% and 90% vertebrae, respectively. The potential of the proposed method is evaluated in an exemplary simulated clinical application.

==> discussion.tex <==
\section{Discussion}

Currently,   clinical   routine   spine   injections   procedures
completely  relies  on  the  expertise  of  the  surgeon,  both  to
ensure the accuracy of the procedure and to limit the exposure  time  to  the  ionizing  radiation. In this study a robotic-ultrasound method for vertebral level detection and counting was developed for spine injections procedure. To  the  best  of  our  knowledge it  is  the  first  robotic  system  integrating  visual  and  force feedback for vertebra level localization. 

The method was tested on a group of healthy volunteers, chosen to maximize the inter-subject variability in terms of gender and BMI. However a more thorough analysis should be conducted in this direction with a larger database. Future exploration should also focus on the online validation of the method in a clinical environment and further automation of each step in the injection procedure. 

In this work, it was proven that the proposed method yielded higher performances compared to pure visual and pure force based methods. The ultrasound-force fusion method was able to correctly classify all the vertebral levels in the test subjects, out-performing the pure-force and pure-image based methods, which could only correctly classify 15 and 17 out of 20 vertebral levels, respectively. Unlike pure-image and pure-force based methods, the performances of the force-ultrasound fusion method do not drop in presence of noise corrupting the ultrasound or force data. In fact, even when one of the two inputs is corrupted, the method can still rely on the un-corrupted data input for the classification task. This can not be performed when only one sensor data is used, where corruption in the input data leads to mis-classification in the output.  

The potential of the proposed method were explored in the integration with a common clinical procedure, opening the path for future exploration toward fully automatic injection procedures.
